The Sixth Moment of Random Determinants for Arbitrarily Distributed Random Entries

Via the method of marked permutation tables presented in this paper, we generalize the formula for the sixth moment of a random determinant to account for entries with arbitrary distribution. That is, let $f_6(n) = \mathbb{E}(\det A)^6$, where $A$ is an $n$ by $n$ random matrix with independent and identically distributed entries. We show that the exponential generating function $F_6(t) = \sum_{n=0}^\infty f_6(n)t^n/(n!)^2$ is D-finite and we present it in a closed form. Our method relies on carefully decomposing marked permutation tables into a shell, a core, and a floating component, each of which has a separate contribution to $F_6(t)$. After this decomposition, it is sufficient to enumerate over a finite number of possible shells, which we did using a highly intricate computer program. We verified our result up to $n = 7$ in the general case and up to $n = 9$ for random matrices whose entries only take two values by using a different method for computing $f_6(n)$ for these cases.

==> D-mark-pattern-tables.tex <==
% Copy/paste-ready appendix for the Overleaf article main.tex.
% All generated symmetry-factor records are inlined below.

\section{Mark-Pattern Tables}
\label{app:mark-pattern-tables}

Here we record the currently selected mark-pattern tables with the symmetry
multiplicity inherited by each partial shell generated from them.  Rows
correspond to the six determinant copies, while columns distinguish
marked-table columns.  A zero denotes an unmarked position.  Equal letters
denote marks covering the same element, and different letters denote
different covered elements.

For a table \(P\), let \(\Aut(P)\) denote its automorphism group.  If
\(\widetilde S\) is a literal partial shell generated from \(P\), let
\(n_{\underline{3}}(\widetilde S)\) be its number of separate
\(\underline{3}\)-columns.  This number is determined by \(P\) and is
constant across its generated descendants in the enumeration convention used
here.  The multiplicity recorded beside \(P\) is therefore
\begin{equation}
  C_{\mathrm{NB}}(P)
    =
  \frac{6!}
       {|\Aut(P)|\,
        n_{\underline{3}}(\widetilde S)!}.
  \label{eq:appendix-mark-table-multiplicity}
\end{equation}
By contrast, \(n_{\underline{4}}(\widetilde S)\), the number of separate
\(\underline{4}\)-columns, is not completely determined by \(P\) and
contributes no factorial to this multiplicity.  The implementation emits
those columns in a prescribed covered-element order, so their permutations
are never generated as distinct records.  Every table below displays the
exact value of
\(C_{\mathrm{NB}}(P)\).


\begingroup
\normalsize
\setlength{\LTpre}{0.9\baselineskip}
\setlength{\LTpost}{1.5\baselineskip}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\newcommand{\marktablefactorrecord}[2]{%
  \scriptstyle C_{\mathrm{NB}}(P)=
  \ifnum#2=1\relax #1\else\frac{#1}{#2}\fi
}
% Generated by code/generate_mark_pattern_multiplicities.py.
% Generator version: mark-pattern-table-multiplicities-v3
% Source SHA-256: 1ccd95ce4bac4186d70c9ae90cd32aa823715db2e39a6877898505e55fd383b1
% Do not edit this file by hand.

\expandafter\def\csname RDMarkFactor@1@1\endcsname{\marktablefactorrecord{6}{1}}
\expandafter\def\csname RDMarkFactor@2@1\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@2@2\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@2@3\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@3@1\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@3@2\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@3@3\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@3@4\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@3@5\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@3@6\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@3@7\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@3@8\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@4@1\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@4@2\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@4@3\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@4\endcsname{\marktablefactorrecord{15}{2}}
\expandafter\def\csname RDMarkFactor@4@5\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@4@6\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@4@7\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@8\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@9\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@10\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@11\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@12\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@4@13\endcsname{\marktablefactorrecord{45}{2}}
\expandafter\def\csname RDMarkFactor@4@14\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@15\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@16\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@4@17\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@4@18\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@19\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@20\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@4@21\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@4@22\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@4@23\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@4@24\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@1\endcsname{\marktablefactorrecord{30}{1}}
\expandafter\def\csname RDMarkFactor@5@2\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@3\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@5@4\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@5@5\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@6\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@7\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@8\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@9\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@10\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@5@11\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@12\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@13\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@14\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@15\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@16\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@17\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@18\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@19\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@20\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@21\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@22\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@23\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@5@24\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@5@25\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@26\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@27\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@28\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@29\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@30\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@31\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@5@32\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@33\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@34\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@35\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@36\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@37\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@38\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@39\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@40\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@41\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@5@42\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@5@43\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@44\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@5@45\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@46\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@5@47\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@5@48\endcsname{\marktablefactorrecord{6}{1}}
\expandafter\def\csname RDMarkFactor@5@49\endcsname{\marktablefactorrecord{30}{1}}
\expandafter\def\csname RDMarkFactor@5@50\endcsname{\marktablefactorrecord{720}{1}}
\expandafter\def\csname RDMarkFactor@5@51\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@1\endcsname{\marktablefactorrecord{1}{1}}
\expandafter\def\csname RDMarkFactor@6@2\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@3\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@4\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@5\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@6\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@7\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@8\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@9\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@10\endcsname{\marktablefactorrecord{10}{1}}
\expandafter\def\csname RDMarkFactor@6@11\endcsname{\marktablefactorrecord{10}{1}}
\expandafter\def\csname RDMarkFactor@6@12\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@13\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@14\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@15\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@16\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@17\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@18\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@19\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@20\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@21\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@22\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@23\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@24\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@25\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@26\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@27\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@28\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@29\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@30\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@31\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@32\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@33\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@34\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@35\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@36\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@37\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@38\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@39\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@40\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@41\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@42\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@43\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@44\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@45\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@46\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@47\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@48\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@49\endcsname{\marktablefactorrecord{720}{1}}
\expandafter\def\csname RDMarkFactor@6@50\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@51\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@52\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@53\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@54\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@55\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@56\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@57\endcsname{\marktablefactorrecord{720}{1}}
\expandafter\def\csname RDMarkFactor@6@58\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@59\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@60\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@61\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@62\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@63\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@64\endcsname{\marktablefactorrecord{10}{1}}
\expandafter\def\csname RDMarkFactor@6@65\endcsname{\marktablefactorrecord{30}{1}}
\expandafter\def\csname RDMarkFactor@6@66\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@67\endcsname{\marktablefactorrecord{30}{1}}
\expandafter\def\csname RDMarkFactor@6@68\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@69\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@70\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@71\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@6@72\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@73\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@74\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@75\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@76\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@77\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@78\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@79\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@6@80\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@81\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@82\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@6@83\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@84\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@85\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@86\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@87\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@88\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@89\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@90\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@91\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@92\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@93\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@94\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@95\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@96\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@97\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@98\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@99\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@100\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@101\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@102\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@103\endcsname{\marktablefactorrecord{720}{1}}
\expandafter\def\csname RDMarkFactor@6@104\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@105\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@106\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@107\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@108\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@109\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@110\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@111\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@112\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@113\endcsname{\marktablefactorrecord{720}{1}}
\expandafter\def\csname RDMarkFactor@6@114\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@115\endcsname{\marktablefactorrecord{15}{2}}
\expandafter\def\csname RDMarkFactor@6@116\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@117\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@118\endcsname{\marktablefactorrecord{15}{2}}
\expandafter\def\csname RDMarkFactor@6@119\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@120\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@121\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@122\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@123\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@124\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@125\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@126\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@127\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@128\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@129\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@130\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@131\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@132\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@133\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@134\endcsname{\marktablefactorrecord{60}{1}}
\expandafter\def\csname RDMarkFactor@6@135\endcsname{\marktablefactorrecord{45}{2}}
\expandafter\def\csname RDMarkFactor@6@136\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@137\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@138\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@139\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@140\endcsname{\marktablefactorrecord{45}{1}}
\expandafter\def\csname RDMarkFactor@6@141\endcsname{\marktablefactorrecord{1}{6}}
\expandafter\def\csname RDMarkFactor@6@142\endcsname{\marktablefactorrecord{5}{2}}
\expandafter\def\csname RDMarkFactor@6@143\endcsname{\marktablefactorrecord{15}{2}}
\expandafter\def\csname RDMarkFactor@6@144\endcsname{\marktablefactorrecord{5}{1}}
\expandafter\def\csname RDMarkFactor@6@145\endcsname{\marktablefactorrecord{30}{1}}
\expandafter\def\csname RDMarkFactor@6@146\endcsname{\marktablefactorrecord{20}{1}}
\expandafter\def\csname RDMarkFactor@6@147\endcsname{\marktablefactorrecord{5}{2}}
\expandafter\def\csname RDMarkFactor@6@148\endcsname{\marktablefactorrecord{45}{2}}
\expandafter\def\csname RDMarkFactor@6@149\endcsname{\marktablefactorrecord{1}{1}}
\expandafter\def\csname RDMarkFactor@6@150\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@151\endcsname{\marktablefactorrecord{360}{1}}
\expandafter\def\csname RDMarkFactor@6@152\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@153\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@154\endcsname{\marktablefactorrecord{90}{1}}
\expandafter\def\csname RDMarkFactor@6@155\endcsname{\marktablefactorrecord{180}{1}}
\expandafter\def\csname RDMarkFactor@6@156\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@157\endcsname{\marktablefactorrecord{15}{1}}
\expandafter\def\csname RDMarkFactor@6@158\endcsname{\marktablefactorrecord{120}{1}}
\expandafter\def\csname RDMarkFactor@6@159\endcsname{\marktablefactorrecord{90}{1}}
\newcommand{\marktableentry}[3]{%
  \(\begin{gathered}
    \mathcal M^{(#1)}_{#2}=
    \left[\begin{smallmatrix}#3\end{smallmatrix}\right]\\[3pt]
    \csname RDMarkFactor@#1@#2\endcsname
  \end{gathered}\)%
}

\Needspace{14\baselineskip}
\subsection{One-mark tables}
\label{sec:mark-pattern-tables-r1}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=1\) mark.}\label{tab:mark-pattern-tables-r1}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{1}{1}{a\\0\\0\\0\\0\\0} &  & \\[16pt]
\end{longtable}

\Needspace{14\baselineskip}
\subsection{Two-mark tables}
\label{sec:mark-pattern-tables-r2}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=2\) marks.}\label{tab:mark-pattern-tables-r2}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{2}{1}{a\\a\\0\\0\\0\\0} & \marktableentry{2}{2}{a\\b\\0\\0\\0\\0} & \marktableentry{2}{3}{a & 0\\0 & b\\0 & 0\\0 & 0\\0 & 0\\0 & 0}\\[16pt]
\end{longtable}

\Needspace{14\baselineskip}
\subsection{Three-mark tables}
\label{sec:mark-pattern-tables-r3}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=3\) marks.}\label{tab:mark-pattern-tables-r3}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{3}{1}{a\\a\\a\\0\\0\\0} & \marktableentry{3}{2}{a\\a\\b\\0\\0\\0} & \marktableentry{3}{3}{a\\b\\c\\0\\0\\0}\\[16pt]
\marktableentry{3}{4}{a & 0\\a & 0\\0 & a\\0 & 0\\0 & 0\\0 & 0} & \marktableentry{3}{5}{a & 0\\a & 0\\0 & b\\0 & 0\\0 & 0\\0 & 0} & \marktableentry{3}{6}{a & 0\\b & 0\\0 & a\\0 & 0\\0 & 0\\0 & 0}\\[16pt]
\marktableentry{3}{7}{a & 0\\b & 0\\0 & c\\0 & 0\\0 & 0\\0 & 0} & \marktableentry{3}{8}{a & 0 & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0\\0 & 0 & 0\\0 & 0 & 0} & \\[16pt]
\end{longtable}

\Needspace{14\baselineskip}
\subsection{Four-mark tables}
\label{sec:mark-pattern-tables-r4}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=4\) marks.}\label{tab:mark-pattern-tables-r4}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{4}{1}{a\\a\\a\\a\\0\\0} & \marktableentry{4}{2}{a\\a\\a\\b\\0\\0} & \marktableentry{4}{3}{a\\a\\b\\c\\0\\0}\\[16pt]
\marktableentry{4}{4}{a\\b\\c\\d\\0\\0} & \marktableentry{4}{5}{a & 0\\a & 0\\0 & a\\0 & a\\0 & 0\\0 & 0} & \marktableentry{4}{6}{a & 0\\a & 0\\0 & b\\0 & b\\0 & 0\\0 & 0}\\[16pt]
\marktableentry{4}{7}{a & 0\\b & 0\\0 & a\\0 & b\\0 & 0\\0 & 0} & \marktableentry{4}{8}{a & 0\\a & 0\\0 & b\\0 & c\\0 & 0\\0 & 0} & \marktableentry{4}{9}{a & 0\\b & 0\\0 & a\\0 & c\\0 & 0\\0 & 0}\\[16pt]
\marktableentry{4}{10}{a & 0\\a & 0\\b & 0\\0 & c\\0 & 0\\0 & 0} & \marktableentry{4}{11}{a & 0\\b & 0\\c & 0\\0 & a\\0 & 0\\0 & 0} & \marktableentry{4}{12}{a & 0\\b & 0\\c & 0\\0 & d\\0 & 0\\0 & 0}\\[16pt]
\marktableentry{4}{13}{a & 0\\b & 0\\0 & c\\0 & d\\0 & 0\\0 & 0} & \marktableentry{4}{14}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0\\0 & 0 & 0} & \marktableentry{4}{15}{a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & 0\\0 & 0 & 0}\\[16pt]
\marktableentry{4}{16}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & 0 & c\\0 & 0 & 0\\0 & 0 & 0} & \marktableentry{4}{17}{a & 0 & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & c\\0 & 0 & 0\\0 & 0 & 0} & \marktableentry{4}{18}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & 0\\0 & 0 & 0}\\[16pt]
\marktableentry{4}{19}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & 0 & a\\0 & 0 & 0\\0 & 0 & 0} & \marktableentry{4}{20}{a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d\\0 & 0 & 0 & 0\\0 & 0 & 0 & 0} & \marktableentry{4}{21}{a & 0\\a & 0\\a & 0\\0 & b\\0 & 0\\0 & 0}\\[16pt]
\marktableentry{4}{22}{a & 0\\a & 0\\b & 0\\0 & a\\0 & 0\\0 & 0} & \marktableentry{4}{23}{a\\a\\b\\b\\0\\0} & \marktableentry{4}{24}{a & 0\\a & 0\\0 & a\\0 & b\\0 & 0\\0 & 0}\\[16pt]
\end{longtable}

\Needspace{14\baselineskip}
\subsection{Five-mark tables}
\label{sec:mark-pattern-tables-r5}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=5\) marks.}\label{tab:mark-pattern-tables-r5}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{5}{1}{a & 0\\a & 0\\a & 0\\a & 0\\0 & b\\0 & 0} & \marktableentry{5}{2}{a & 0\\a & 0\\0 & a\\0 & a\\0 & b\\0 & 0} & \marktableentry{5}{3}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{4}{a & 0\\a & 0\\a & 0\\b & 0\\0 & a\\0 & 0} & \marktableentry{5}{5}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & 0} & \marktableentry{5}{6}{a & 0\\a & 0\\a & 0\\0 & b\\0 & b\\0 & 0}\\[16pt]
\marktableentry{5}{7}{a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & b\\0 & 0 & 0} & \marktableentry{5}{8}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & 0} & \marktableentry{5}{9}{a & 0\\a & 0\\b & 0\\b & 0\\0 & a\\0 & 0}\\[16pt]
\marktableentry{5}{10}{a & 0\\a & 0\\a & 0\\b & 0\\0 & c\\0 & 0} & \marktableentry{5}{11}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0} & \marktableentry{5}{12}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{13}{a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & a & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & c\\0 & 0 & 0 & 0} & \marktableentry{5}{14}{a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0} & \marktableentry{5}{15}{a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & a & 0\\0 & 0 & b & 0\\0 & 0 & 0 & c\\0 & 0 & 0 & 0}\\[16pt]
\marktableentry{5}{16}{a & 0\\a & 0\\a & 0\\0 & b\\0 & c\\0 & 0} & \marktableentry{5}{17}{a & 0\\a & 0\\b & 0\\0 & a\\0 & c\\0 & 0} & \marktableentry{5}{18}{a & 0\\a & 0\\b & 0\\c & 0\\0 & b\\0 & 0}\\[16pt]
\marktableentry{5}{19}{a & 0\\a & 0\\0 & a\\0 & b\\0 & c\\0 & 0} & \marktableentry{5}{20}{a & 0\\0 & a\\0 & a\\0 & b\\0 & c\\0 & 0} & \marktableentry{5}{21}{a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & c\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{22}{a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b\\0 & 0 & 0 & c\\0 & 0 & 0 & 0} & \marktableentry{5}{23}{a & 0\\a & 0\\b & 0\\b & 0\\0 & c\\0 & 0} & \marktableentry{5}{24}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{25}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & 0} & \marktableentry{5}{26}{a & 0 & 0\\0 & a & 0\\0 & 0 & a\\0 & 0 & b\\0 & 0 & c\\0 & 0 & 0} & \marktableentry{5}{27}{a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & c\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{28}{a & 0\\a & 0\\c & 0\\0 & b\\0 & b\\0 & 0} & \marktableentry{5}{29}{a & 0\\b & 0\\c & 0\\0 & a\\0 & b\\0 & 0} & \marktableentry{5}{30}{a & 0\\a & 0\\b & 0\\c & 0\\0 & d\\0 & 0}\\[16pt]
\marktableentry{5}{31}{a & 0\\b & 0\\c & 0\\d & 0\\0 & a\\0 & 0} & \marktableentry{5}{32}{a & 0\\b & 0\\c & 0\\0 & a\\0 & d\\0 & 0} & \marktableentry{5}{33}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{34}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & 0} & \marktableentry{5}{35}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & 0} & \marktableentry{5}{36}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & 0 & d\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{37}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d\\0 & 0 & 0 & 0} & \marktableentry{5}{38}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d\\0 & 0 & 0 & 0} & \marktableentry{5}{39}{a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & b & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d\\0 & 0 & 0 & 0}\\[16pt]
\marktableentry{5}{40}{a & 0\\a & 0\\0 & b\\0 & c\\0 & d\\0 & 0} & \marktableentry{5}{41}{a & 0\\a & 0\\b & 0\\0 & c\\0 & d\\0 & 0} & \marktableentry{5}{42}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & 0 & c\\0 & 0 & d\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{43}{a & 0 & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & c\\0 & 0 & d\\0 & 0 & 0} & \marktableentry{5}{44}{a & 0\\b & 0\\c & 0\\d & 0\\0 & e\\0 & 0} & \marktableentry{5}{45}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & d & 0\\0 & 0 & e\\0 & 0 & 0}\\[16pt]
\marktableentry{5}{46}{a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & d & 0\\0 & 0 & e\\0 & 0 & 0} & \marktableentry{5}{47}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & c & 0 & 0\\0 & 0 & d & 0\\0 & 0 & 0 & e\\0 & 0 & 0 & 0} & \marktableentry{5}{48}{a & 0 & 0 & 0 & 0\\0 & b & 0 & 0 & 0\\0 & 0 & c & 0 & 0\\0 & 0 & 0 & d & 0\\0 & 0 & 0 & 0 & e\\0 & 0 & 0 & 0 & 0}\\[16pt]
\marktableentry{5}{49}{a & 0\\b & 0\\c & 0\\0 & d\\0 & e\\0 & 0} & \marktableentry{5}{50}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & b\\0 & 0 & 0} & \marktableentry{5}{51}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & b\\0 & 0 & 0}\\[16pt]
\end{longtable}

\Needspace{14\baselineskip}
\subsection{Six-mark tables}
\label{sec:mark-pattern-tables-r6}

\begin{longtable}{@{}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}>{\centering\arraybackslash}p{0.31\textwidth}@{}}
\caption{Mark-pattern tables with \(r=6\) marks.}\label{tab:mark-pattern-tables-r6}\\
\toprule
\endfirsthead
\toprule
\endhead
\bottomrule
\endfoot
\marktableentry{6}{1}{a\\a\\a\\a\\a\\a} & \marktableentry{6}{2}{a & 0\\a & 0\\a & 0\\a & 0\\0 & a\\0 & a} & \marktableentry{6}{3}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & a\\0 & 0 & a}\\[16pt]
\marktableentry{6}{4}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & b} & \marktableentry{6}{5}{a & 0\\a & 0\\a & 0\\a & 0\\0 & b\\0 & b} & \marktableentry{6}{6}{a & 0\\a & 0\\b & 0\\b & 0\\0 & a\\0 & a}\\[16pt]
\marktableentry{6}{7}{a\\a\\a\\a\\b\\b} & \marktableentry{6}{8}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & a} & \marktableentry{6}{9}{a & 0\\a & 0\\a & 0\\b & 0\\0 & a\\0 & b}\\[16pt]
\marktableentry{6}{10}{a\\a\\a\\b\\b\\b} & \marktableentry{6}{11}{a & 0\\a & 0\\a & 0\\0 & b\\0 & b\\0 & b} & \marktableentry{6}{12}{a & 0\\a & 0\\a & 0\\b & 0\\0 & b\\0 & b}\\[16pt]
\marktableentry{6}{13}{a & 0\\a & 0\\b & 0\\b & 0\\0 & a\\0 & b} & \marktableentry{6}{14}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & b} & \marktableentry{6}{15}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & b}\\[16pt]
\marktableentry{6}{16}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\b & 0 & 0\\0 & b & 0\\0 & 0 & a} & \marktableentry{6}{17}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & b} & \marktableentry{6}{18}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & b & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b}\\[16pt]
\marktableentry{6}{19}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & b & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b} & \marktableentry{6}{20}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & 0 & c} & \marktableentry{6}{21}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & 0 & c}\\[16pt]
\marktableentry{6}{22}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & 0 & a} & \marktableentry{6}{23}{a\\a\\a\\a\\b\\c} & \marktableentry{6}{24}{a & 0\\a & 0\\a & 0\\a & 0\\0 & b\\0 & c}\\[16pt]
\marktableentry{6}{25}{a & 0\\a & 0\\a & 0\\b & 0\\0 & a\\0 & c} & \marktableentry{6}{26}{a & 0\\a & 0\\b & 0\\c & 0\\0 & a\\0 & a} & \marktableentry{6}{27}{a & 0\\a & 0\\b & 0\\0 & a\\0 & a\\0 & c}\\[16pt]
\marktableentry{6}{28}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & a} & \marktableentry{6}{29}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & c} & \marktableentry{6}{30}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & a}\\[16pt]
\marktableentry{6}{31}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & b\\0 & 0 & c} & \marktableentry{6}{32}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & c} & \marktableentry{6}{33}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & a & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & c}\\[16pt]
\marktableentry{6}{34}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & b & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & c} & \marktableentry{6}{35}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a} & \marktableentry{6}{36}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a}\\[16pt]
\marktableentry{6}{37}{a\\a\\a\\b\\b\\c} & \marktableentry{6}{38}{a & 0\\a & 0\\a & 0\\b & 0\\0 & b\\0 & c} & \marktableentry{6}{39}{a & 0\\a & 0\\b & 0\\b & 0\\0 & a\\0 & c}\\[16pt]
\marktableentry{6}{40}{a & 0\\a & 0\\b & 0\\c & 0\\0 & a\\0 & b} & \marktableentry{6}{41}{a & 0\\a & 0\\a & 0\\c & 0\\0 & b\\0 & b} & \marktableentry{6}{42}{a & 0\\b & 0\\b & 0\\c & 0\\0 & a\\0 & a}\\[16pt]
\marktableentry{6}{43}{a & 0\\a & 0\\a & 0\\0 & b\\0 & b\\0 & c} & \marktableentry{6}{44}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & 0 & c} & \marktableentry{6}{45}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & 0 & b}\\[16pt]
\marktableentry{6}{46}{a & 0 & 0\\b & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & 0 & a} & \marktableentry{6}{47}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & c} & \marktableentry{6}{48}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & b}\\[16pt]
\marktableentry{6}{49}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a} & \marktableentry{6}{50}{b & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & a} & \marktableentry{6}{51}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & b\\0 & 0 & c}\\[16pt]
\marktableentry{6}{52}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & c} & \marktableentry{6}{53}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & a\\0 & 0 & c} & \marktableentry{6}{54}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & b & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & c}\\[16pt]
\marktableentry{6}{55}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & b & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & c} & \marktableentry{6}{56}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b} & \marktableentry{6}{57}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b}\\[16pt]
\marktableentry{6}{58}{a\\a\\b\\b\\c\\c} & \marktableentry{6}{59}{a & 0\\a & 0\\b & 0\\b & 0\\0 & c\\0 & c} & \marktableentry{6}{60}{a & 0\\a & 0\\b & 0\\c & 0\\0 & b\\0 & c}\\[16pt]
\marktableentry{6}{61}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & c} & \marktableentry{6}{62}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & c} & \marktableentry{6}{63}{a & 0 & 0\\b & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & a\\0 & 0 & c}\\[16pt]
\marktableentry{6}{64}{a\\a\\a\\b\\c\\d} & \marktableentry{6}{65}{a & 0\\a & 0\\a & 0\\b & 0\\0 & c\\0 & d} & \marktableentry{6}{66}{a & 0\\a & 0\\b & 0\\c & 0\\0 & a\\0 & d}\\[16pt]
\marktableentry{6}{67}{a & 0\\b & 0\\c & 0\\d & 0\\0 & a\\0 & a} & \marktableentry{6}{68}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & 0 & d} & \marktableentry{6}{69}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & 0 & d}\\[16pt]
\marktableentry{6}{70}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & 0 & a} & \marktableentry{6}{71}{a & 0\\a & 0\\a & 0\\0 & b\\0 & c\\0 & d} & \marktableentry{6}{72}{a & 0\\a & 0\\b & 0\\0 & a\\0 & c\\0 & d}\\[16pt]
\marktableentry{6}{73}{a & 0 & 0\\a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & d} & \marktableentry{6}{74}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & d} & \marktableentry{6}{75}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & d & 0\\0 & 0 & a}\\[16pt]
\marktableentry{6}{76}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & d} & \marktableentry{6}{77}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & d & 0\\0 & 0 & a} & \marktableentry{6}{78}{b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & a}\\[16pt]
\marktableentry{6}{79}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d} & \marktableentry{6}{80}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d} & \marktableentry{6}{81}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & d}\\[16pt]
\marktableentry{6}{82}{b & 0 & 0 & 0\\c & 0 & 0 & 0\\d & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a} & \marktableentry{6}{83}{a & 0 & 0\\a & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & d} & \marktableentry{6}{84}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & a\\0 & 0 & d}\\[16pt]
\marktableentry{6}{85}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & a & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d} & \marktableentry{6}{86}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & d} & \marktableentry{6}{87}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & d}\\[16pt]
\marktableentry{6}{88}{b & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & a & 0 & 0\\0 & d & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a} & \marktableentry{6}{89}{a\\a\\b\\b\\c\\d} & \marktableentry{6}{90}{a & 0\\a & 0\\b & 0\\b & 0\\0 & c\\0 & d}\\[16pt]
\marktableentry{6}{91}{a & 0\\a & 0\\b & 0\\c & 0\\0 & b\\0 & d} & \marktableentry{6}{92}{a & 0\\a & 0\\c & 0\\d & 0\\0 & b\\0 & b} & \marktableentry{6}{93}{a & 0\\b & 0\\c & 0\\d & 0\\0 & a\\0 & b}\\[16pt]
\marktableentry{6}{94}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & 0 & d} & \marktableentry{6}{95}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & b & 0\\0 & 0 & d} & \marktableentry{6}{96}{a & 0 & 0\\a & 0 & 0\\d & 0 & 0\\c & 0 & 0\\0 & b & 0\\0 & 0 & b}\\[16pt]
\marktableentry{6}{97}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & 0 & b} & \marktableentry{6}{98}{a & 0\\a & 0\\c & 0\\0 & b\\0 & b\\0 & d} & \marktableentry{6}{99}{a & 0\\b & 0\\c & 0\\0 & a\\0 & b\\0 & d}\\[16pt]
\marktableentry{6}{100}{a & 0 & 0\\a & 0 & 0\\c & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & d} & \marktableentry{6}{101}{a & 0 & 0\\a & 0 & 0\\c & 0 & 0\\0 & b & 0\\0 & d & 0\\0 & 0 & b} & \marktableentry{6}{102}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & d}\\[16pt]
\marktableentry{6}{103}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & d & 0\\0 & 0 & b} & \marktableentry{6}{104}{a & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & a} & \marktableentry{6}{105}{a & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & b}\\[16pt]
\marktableentry{6}{106}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & d} & \marktableentry{6}{107}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & b\\0 & 0 & d} & \marktableentry{6}{108}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & b\\0 & 0 & d}\\[16pt]
\marktableentry{6}{109}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d} & \marktableentry{6}{110}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & c & 0 & 0\\0 & d & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & b} & \marktableentry{6}{111}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & c & 0 & 0\\0 & d & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & d}\\[16pt]
\marktableentry{6}{112}{a & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & a & 0 & 0\\0 & d & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & b} & \marktableentry{6}{113}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & b & 0\\0 & 0 & 0 & d} & \marktableentry{6}{114}{a & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & b & 0 & 0\\0 & d & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b}\\[16pt]
\marktableentry{6}{115}{a\\a\\b\\c\\d\\e} & \marktableentry{6}{116}{a & 0\\a & 0\\b & 0\\c & 0\\0 & d\\0 & e} & \marktableentry{6}{117}{a & 0\\b & 0\\c & 0\\d & 0\\0 & a\\0 & e}\\[16pt]
\marktableentry{6}{118}{b & 0\\c & 0\\d & 0\\e & 0\\0 & a\\0 & a} & \marktableentry{6}{119}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & d & 0\\0 & 0 & e} & \marktableentry{6}{120}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & 0 & e}\\[16pt]
\marktableentry{6}{121}{b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\e & 0 & 0\\0 & a & 0\\0 & 0 & a} & \marktableentry{6}{122}{a & 0\\a & 0\\b & 0\\0 & c\\0 & d\\0 & e} & \marktableentry{6}{123}{a & 0\\b & 0\\c & 0\\0 & a\\0 & d\\0 & e}\\[16pt]
\marktableentry{6}{124}{a & 0 & 0\\a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & d & 0\\0 & 0 & e} & \marktableentry{6}{125}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & a & 0\\0 & d & 0\\0 & 0 & e} & \marktableentry{6}{126}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & d & 0\\0 & e & 0\\0 & 0 & a}\\[16pt]
\marktableentry{6}{127}{b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & a & 0\\0 & 0 & e} & \marktableentry{6}{128}{b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & a & 0\\0 & e & 0\\0 & 0 & a} & \marktableentry{6}{129}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & c & 0 & 0\\0 & 0 & d & 0\\0 & 0 & 0 & e}\\[16pt]
\marktableentry{6}{130}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & d & 0\\0 & 0 & 0 & e} & \marktableentry{6}{131}{b & 0 & 0 & 0\\c & 0 & 0 & 0\\d & 0 & 0 & 0\\0 & a & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & e} & \marktableentry{6}{132}{a & 0 & 0 & 0 & 0\\a & 0 & 0 & 0 & 0\\0 & a & 0 & 0 & 0\\0 & 0 & b & 0 & 0\\0 & 0 & 0 & c & 0\\0 & 0 & 0 & 0 & d}\\[16pt]
\marktableentry{6}{133}{a & 0 & 0 & 0 & 0\\b & 0 & 0 & 0 & 0\\0 & a & 0 & 0 & 0\\0 & 0 & a & 0 & 0\\0 & 0 & 0 & c & 0\\0 & 0 & 0 & 0 & d} & \marktableentry{6}{134}{b & 0 & 0 & 0 & 0\\c & 0 & 0 & 0 & 0\\0 & a & 0 & 0 & 0\\0 & 0 & a & 0 & 0\\0 & 0 & 0 & a & 0\\0 & 0 & 0 & 0 & d} & \marktableentry{6}{135}{a & 0 & 0\\a & 0 & 0\\0 & b & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & e}\\[16pt]
\marktableentry{6}{136}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & c & 0\\0 & 0 & d\\0 & 0 & e} & \marktableentry{6}{137}{a & 0 & 0 & 0\\a & 0 & 0 & 0\\0 & b & 0 & 0\\0 & c & 0 & 0\\0 & 0 & d & 0\\0 & 0 & 0 & e} & \marktableentry{6}{138}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & d & 0\\0 & 0 & 0 & e}\\[16pt]
\marktableentry{6}{139}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & c & 0 & 0\\0 & d & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & e} & \marktableentry{6}{140}{b & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & d & 0 & 0\\0 & e & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a} & \marktableentry{6}{141}{a\\b\\c\\d\\e\\f}\\[16pt]
\marktableentry{6}{142}{a & 0\\b & 0\\c & 0\\d & 0\\0 & e\\0 & f} & \marktableentry{6}{143}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\d & 0 & 0\\0 & e & 0\\0 & 0 & f} & \marktableentry{6}{144}{a & 0\\b & 0\\c & 0\\0 & d\\0 & e\\0 & f}\\[16pt]
\marktableentry{6}{145}{a & 0 & 0\\b & 0 & 0\\c & 0 & 0\\0 & d & 0\\0 & e & 0\\0 & 0 & f} & \marktableentry{6}{146}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\c & 0 & 0 & 0\\0 & d & 0 & 0\\0 & 0 & e & 0\\0 & 0 & 0 & f} & \marktableentry{6}{147}{a & 0 & 0\\b & 0 & 0\\0 & c & 0\\0 & d & 0\\0 & 0 & e\\0 & 0 & f}\\[16pt]
\marktableentry{6}{148}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & c & 0 & 0\\0 & d & 0 & 0\\0 & 0 & e & 0\\0 & 0 & 0 & f} & \marktableentry{6}{149}{a & 0 & 0 & 0 & 0 & 0\\0 & b & 0 & 0 & 0 & 0\\0 & 0 & c & 0 & 0 & 0\\0 & 0 & 0 & d & 0 & 0\\0 & 0 & 0 & 0 & e & 0\\0 & 0 & 0 & 0 & 0 & f} & \marktableentry{6}{150}{b & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a}\\[16pt]
\marktableentry{6}{151}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & b & 0 & 0\\0 & c & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & a} & \marktableentry{6}{152}{a & 0 & 0\\a & 0 & 0\\c & 0 & 0\\0 & b & 0\\0 & b & 0\\0 & 0 & a} & \marktableentry{6}{153}{a & 0 & 0\\b & 0 & 0\\0 & a & 0\\0 & b & 0\\0 & 0 & c\\0 & 0 & d}\\[16pt]
\marktableentry{6}{154}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & a & 0 & 0\\0 & b & 0 & 0\\0 & 0 & c & 0\\0 & 0 & 0 & d} & \marktableentry{6}{155}{a & 0 & 0 & 0\\b & 0 & 0 & 0\\0 & c & 0 & 0\\0 & d & 0 & 0\\0 & 0 & a & 0\\0 & 0 & 0 & b} & \marktableentry{6}{156}{a & 0 & 0 & 0 & 0\\b & 0 & 0 & 0 & 0\\0 & c & 0 & 0 & 0\\0 & 0 & d & 0 & 0\\0 & 0 & 0 & e & 0\\0 & 0 & 0 & 0 & f}\\[16pt]
\marktableentry{6}{157}{a & 0 & 0 & 0 & 0\\a & 0 & 0 & 0 & 0\\0 & b & 0 & 0 & 0\\0 & 0 & c & 0 & 0\\0 & 0 & 0 & d & 0\\0 & 0 & 0 & 0 & e} & \marktableentry{6}{158}{a & 0 & 0 & 0 & 0\\b & 0 & 0 & 0 & 0\\0 & a & 0 & 0 & 0\\0 & 0 & c & 0 & 0\\0 & 0 & 0 & d & 0\\0 & 0 & 0 & 0 & e} & \marktableentry{6}{159}{b & 0 & 0 & 0 & 0\\c & 0 & 0 & 0 & 0\\0 & a & 0 & 0 & 0\\0 & 0 & a & 0 & 0\\0 & 0 & 0 & d & 0\\0 & 0 & 0 & 0 & e}\\[16pt]
\end{longtable}

\endgroup

